Learning to Focus: Causal Attention Distillation via Gradient-Guided Token Pruning

Large language models (LLMs) have demonstrated significant improvements in contextual understanding. However, their ability to attend to truly critical information during long-context reasoning and generation still falls behind the pace. Specifically, our preliminary experiments reveal that certain distracting patterns can misdirect the model's attention during inference, and removing these patterns substantially improves reasoning accuracy and generation quality. We attribute this phenomenon to spurious correlations in the training data, which obstruct the model's capacity to infer authentic causal instruction-response relationships. This phenomenon may induce redundant reasoning processes, potentially resulting in significant inference overhead and, more critically, the generation of erroneous or suboptimal responses. To mitigate this, we introduce a two-stage framework called Learning to Focus (LeaF) leveraging intervention-based inference to disentangle confounding factors. In the first stage, LeaF employs gradient-based comparisons with an advanced teacher to automatically identify confounding tokens based on causal relationships in the training corpus. Then, in the second stage, it prunes these tokens during distillation to enact intervention, aligning the student's attention with the teacher's focus distribution on truly critical context tokens. Experimental results demonstrate that LeaF not only achieves an absolute improvement in various mathematical reasoning, code generation and multi-hop question answering benchmarks but also effectively suppresses attention to confounding tokens during inference, yielding a more interpretable and reliable reasoning model.

==> hhcfmqnhvcmhjgxhytsngfvvpqzcbcgv/prompts/evaluation_code_prompt.tex <==
\begin{prompt}{Evaluation Prompt}
\label{prompt: evaluation_prompt}
The following is a math problem and a solution.
\\
The solution is presented as a step-by-step chain of thought.
\\
Each step is separated with the index indicator ``Step i:'', with i indexed starting from 1.
\\
\\
<Problem>
\\
\{problem\}
\\
</Problem>
\\
\\
<Solution>
\\
\{tagged\_response\}
\\
</Solution>
\\
\\
Your task is to evaluate the solution and identify the earliest step that contains an error, or confirm that all steps are correct.
\\
Please first review and generate a critique for each step.
\\
After reviewing each step, once you identify an error in the step, stop the critique and return the index of that step as this is the step where the earliest error occurs. Otherwise, continue reviewing the subsequent steps. If all steps are correct, return the index of -1 (which typically denotes ``not found'').
\\
Finally, put your final answer (i.e., the step index) in \verb|\|boxed\{\}.
\end{prompt}

==> hhcfmqnhvcmhjgxhytsngfvvpqzcbcgv/sections/01_abstract.tex <==
%==
Large language models (LLMs) have demonstrated significant improvements in contextual understanding. 
%==
However, their ability to attend to truly critical information during long-context reasoning and generation still falls behind the pace.
%==
Specifically, our preliminary experiments reveal that certain distracting patterns can misdirect the model’s attention during inference, and removing these patterns substantially improves reasoning accuracy and generation quality.
%=
We attribute this phenomenon to spurious correlations in the training data, which obstruct the model’s capacity to infer authentic causal instruction–response relationships. 
%==
This phenomenon may induce redundant reasoning processes, potentially resulting in significant inference overhead and, more critically, the generation of erroneous or suboptimal responses.
%==
To mitigate this, we introduce a two-stage framework called \textbf{Lea}rning to \textbf{F}ocus \textbf{(LeaF)} leveraging intervention-based inference to disentangle confounding factors.
%=
In the first stage, LeaF employs gradient-based comparisons with an advanced teacher to automatically identify confounding tokens based on causal relationships in the training corpus. 
%=
Then, in the second stage, it prunes these tokens during distillation to enact intervention, aligning the student’s attention with the teacher’s focus distribution on truly critical context tokens.
%=
Experimental results demonstrate that LeaF not only achieves an absolute improvement in various mathematical reasoning, code generation and multi-hop question answering benchmarks but also effectively suppresses attention to confounding tokens during inference, yielding a more interpretable and reliable reasoning model.
\footnote{Code and data are available at \url{https://github.com/RUCBM/LeaF}.}



==> hhcfmqnhvcmhjgxhytsngfvvpqzcbcgv/sections/02_introduction.tex <==
\section{Introduction}
\begin{figure}[t]
  \centering
  \subfigure[Code Accuracy Improvement]{
    \includegraphics[width=0.45\textwidth]{Figures/code_acc.pdf}
    \label{fig:code_acc}
  }
  \hfill
  \subfigure[MATH Accuracy Improvement]{
    \includegraphics[width=0.45\textwidth]{Figures/math_acc.pdf}
    \label{fig:math_acc}
  }
  \caption{Accuracy improvements achieved by removing confounding tokens from small models on the math and code training corpora. The results demonstrate a significant increase in performance, with over 20\% improvement on the math corpus and more than 10\% on the code corpus. (For further details on these categories, see Appendix~\ref{apex: pre-examination}.)}
  \label{fig:accuracy_delete_misleading}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\textwidth]{Figures/misleading_example.pdf} % 修改路径为你的图片路径
    \caption{Comparison of reasoning before and after pruning distracting patterns. \textcolor{blue}{Blue-shaded regions} indicate pruned confounding tokens. \textcolor{pink}{Pink highlights} mark areas that require focus, while \textcolor{blue}{blue highlights} show where excessive attention caused errors. 
    % Removing distracting patterns from the instruction, without additional training, helps the model focus on critical information and enhance reasoning. This suggests that improving attention to relevant details is a promising direction for advancing model reasoning.
    }
    \label{fig:example}
    \vspace{-0.4cm}
\end{figure}



Large language models (LLMs) have achieved remarkable success in natural language processing tasks, demonstrating strong capabilities in contextual understanding~\citep{zhao2024enhancing,nam2024using,an2024make} and language generation~\citep{gatt2018survey,dong2022survey}. Despite these advancements, LLMs still struggle to maintain focus on truly critical information, especially in long-context reasoning~\citep{yen2024helmet,zhang2024infty,hsieh2024ruler} and complex instruction-based tasks~\citep{ye2025longproc,ling2025longreason}, which adversely impacts reasoning accuracy and generation quality.

%=
% Our preliminary experiments reveal that current LLMs are often influenced by distracting information, leading to erroneous responses. 
%=
% To quantify this effect,
To systematically investigate this phenomenon, we first identify distracting patterns via gradient-based comparisons of teacher and student sensitivities, then assess the performance of student models on NuminaMath-CoT~\cite{numina_math_datasets} and AceCode-87K~\cite{AceCoder}.
% Specifically, to explore how consistency influences reasoning in language models, we identify distracting patterns via gradient-based comparisons and quantify the impact of their removal on small model accuracy across NuminaMath-CoT~\cite{numina_math_datasets} and AceCode-87K~\cite{AceCoder}. 
%=
Surprisingly, as shown in Figure~\ref{fig:accuracy_delete_misleading}, simply pruning distracting patterns yields substantial gains—improving average accuracy by over 20\% on the MATH training corpus~\cite{numina_math_datasets} and more than 10\% on Code training corpus~\cite{AceCoder}. 
%=
% As question difficulty increases (e.g., in AMC\_AIME and Olympiads~\cite{numina_math_datasets} settings), distracting patterns further divert attention from critical reasoning signals. 
Furthermore, we observe greater improvements on AMC\_AIME~\cite{numina_math_datasets} compared to GSM8K~\cite{cobbe2021gsm8k}, suggesting that complex reasoning problems may contain more distracting patterns that interfere with model inference.
%=
These findings demonstrate that mitigating the influence of distracting patterns is essential for improving the robustness and accuracy of LLM reasoning.
% We attribute this improvement to the model's limited capacity to focus on critical information in complex contexts. 
%=
% As question difficulty increases (e.g., in AMC\_AIME and Olympiads~\cite{numina_math_datasets} settings), distracting patterns further divert attention from critical reasoning signals. 
%=
% We further present a representative case in Figure~\ref{fig:example} to illustrate how LLMs can benefit from removing distracting patterns.
We further present a representative case in Figure~\ref{fig:example}.
Removing distracting patterns from the
instruction, without any additional training, helps the model focus on critical information and enhance reasoning. This suggests that improving attention to relevant details is a promising direction for
advancing model reasoning.
% These results underscore the importance of identifying and mitigating spurious confounders to unlock LLMs’ latent reasoning potential.
% These results suggest that identifying and mitigating such distractions is essential to unlocking the model’s latent reasoning potential.
%=

% Based on these analyses, we adopt a causal perspective (Figure~\ref{fig:causal_graph}) to explain and mitigate the observed phenomenon. We treat distracting patterns as spurious confounders in the reasoning process and propose Learning to Focus (LeaF), a two-stage framework that disentangles spurious correlations and refines attention mechanisms in LLMs.
% %=
% In the first stage, LeaF identifies potential spurious confounders by comparing gradient sensitivities between a teacher and a student model.
%=
Based on our analysis, we adopt a causal perspective (Figure~\ref{fig:causal_graph}) to explain and mitigate the observed phenomenon. We propose \textbf{Learning to Focus} (\textbf{LeaF}), a two-stage framework that treats distracting patterns as spurious confounders in LLM reasoning.
In the first stage, LeaF identifies confounding tokens through gradient-based comparisons between a high-capacity teacher and a student model.
Then, it generates counterfactual samples by span pruning, removing contiguous spans of the detected confounding tokens from each instruction.
% Then it performs span pruning and data augmentation to create counterfactual instruction variants. 
In the second stage, LeaF introduces a hybrid distillation loss that minimizes two KL divergences: one for original sample (standard distillation) and one for counterfactual sample (counterfactual distillation). 
This composite objective encourages the student model to capture true causal dependencies by contrasting the teacher model’s outputs before and after pruning confounding tokens, improving the robustness and interpretability of LLM reasoning.


We demonstrate through comprehensive experiments that Learning to Focus (LeaF) significantly enhances critical token identification and attention consistency during inference, leading to improved performance on downstream tasks such as mathematical reasoning, code generation and multi-hop question answering.
%=
Compared to standard knowledge distillation,
%=
LeaF yields an average accuracy gain of 2.41\% on GSM8K~\cite{cobbe2021gsm8k}, MATH-500~\cite{math_benchmark}, and OlympiadBench~\cite{he2024olympiadbench} for LLaMA-1B/3B-Instruct~\cite{liu2024llama3b} and Qwen2.5-Math-1.5B~\cite{yang2024qwen2}. 
In code generation, LeaF achieves an average improvement of 2.48\% on HumanEval+~\cite{evalplus}, LeetCode~\cite{leetcode} and LivecodeBench~\cite{jain2024livecodebench}.
On multi-hop question answering, LeaF improves performance by an average of 3.24\% on HotpotQA~\cite{yang2018hotpotqa}, 2WikiMultiHopQA~\cite{ho2020constructing}, and Musique~\cite{trivedi2022musique}.
%=
These results validate our hypothesis that enhancing attention to key information is critical for improving reasoning performance. 
Attention visualizations in Section~\ref{sec:case_study} further demonstrate LeaF’s interpretability.


==> hhcfmqnhvcmhjgxhytsngfvvpqzcbcgv/sections/03_method.tex <==
\section{Methodology}
\subsection{Causal Framework}

Following Pearl's Structural Causal Model~\cite{pearl2010causal}, we formulate a DAG $G$ to model the causal relationships among different components (refer to Figure~\ref{fig:causal_graph}). We assume the distribution of $(X, A, Y)$ is faithful to the DAG. In this framework,  \( X = [x_1, x_2, \dots, x_n] \) represents the input tokens, and $Y$ is the model's output. Confounding tokens, denoted as $A$, are a subset of $X$ that introduce spurious correlations during reasoning. Unlike regular tokens that convey semantic information, confounding tokens hide the true causal relationship, leading to incorrect predictions. To better understand the DAG, we construct two hypotheses to describe the influence of confounding tokens $A$ on the generation process of $Y$:
\begin{wrapfigure}{r}{0.48\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{Figures/Causal_graph.pdf}
\setlength{\abovecaptionskip}{-0.8em}  
    \caption{Causal graph of the reasoning process. $X$ represents the input prompt, and $Y$ denotes the model's output. A subset of tokens in $X$, identified as confounding tokens ($A$), introduces spurious correlations that disrupt the reasoning process. Our method detects and masks $A$, effectively eliminating the spurious edge from $A$ to $Y$ and restoring the true causal dependency.}
    \label{fig:causal_graph}
    \vspace{-1.18cm}  
\end{wrapfigure}
\paragraph{$\mathcal{H}_0$: There is no causal edge from $A$ to $Y$.}
In this scenario, $A$ does not interfere with the generation of $Y$, and the model's reasoning path is purely determined by the meaningful tokens in $X \setminus A$. Formally, $A$ and $Y$ are \textbf{d-separated}
given $X \setminus A$, 
% (i.e., all paths from any token in \(A\) to \(Y\) are blocked once we condition on \(X \setminus A\))
which implies:
\begin{equation}
    P(Y \mid X) = P(Y \mid X \setminus A).
\end{equation}

% \paragraph{$\mathcal{H}_1$: There is a spurious correlation between $A$ to $Y$.}
\paragraph{$\mathcal{H}_1$: There is a nonzero causal edge from \(A\) to \(Y\).}
Equivalently, \(A\) and \(Y\) are not d-separated given \(X \setminus A\), which implies
\[
P(Y \mid X) \;\neq\; P\bigl(Y \mid X \setminus A\bigr).
\]
In this case, $A$ interfere with the output $Y$ by introducing erroneous correlations. This spurious dependency not only distorts the model's attention but also biases its output, leading to unreliable predictions.

% \subsection{d-Separation and Causal Inference}

The desired behavior of the model is to \textbf{remove the spurious correlation} of $A$ on $Y$, which corresponds to $\mathcal{H}_0$. To achieve this, we utilize the following d-separation properties in the DAG $G$:

\paragraph{R1: Under $\mathcal{H}_0$, $A$ and $Y$ are d-separated by $X \setminus A$.}
This implies that, conditional on the meaningful tokens in $X$, the confounding tokens $A$ should have no direct or indirect effect on $Y$:
\begin{equation}
    A \perp Y \mid (X \setminus A).
\end{equation}

\paragraph{R2: Under $\mathcal{H}_1$, $A$ and $Y$ are not d-separated by $X$, leading to spurious influences.}
In traditional LLM reasoning, these spurious paths can be exploited, causing the model to rely on distracting patterns. To eliminate this dependency, our method introduces \textbf{causal pruning}, effectively removing the influence of $A$ before distillation. This enables the distillation process to focus on the true causal pathways, refining the attention mechanism in the student model.

\subsection{\texttt{LeaF}: Learning to Focus Framework}
\label{sec:LeaF}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\textwidth]{Figures/main_.pdf} % 修改路径为你的图片路径
    \caption{\textbf{Method Overview.} The training pipeline comprises two key stages: (1) \textbf{Confounding Token Detection}: gradient-based comparisons between an advanced teacher model and the student model are used to identify confounding tokens (confounders) in the training corpus; and (2) \textbf{Causal Attention Distillation}: prune identified confounders respectively during training to align the student’s attention with the teacher’s and capture casual relationships. This targeted intervention steers the model toward actual causal dependencies, enhancing both robustness and interpretability.}
    \label{fig:main}
    \vspace{-0.3cm}
\end{figure}

To achieve the desired d-separation and eliminate spurious dependencies, we introduce a \textbf{Learning to Focus Framework (LeaF)} (Figure ~\ref{fig:main}), which consists of two main stages:  
(1) Confounding Token Detection (Section~\ref{misleading_tokens_detection}) and (2) Causal Attention Distillation (Section~\ref{causal_attention}). We discuss them in detail in the following.

\subsubsection{Confounding Token Detection} \label{misleading_tokens_detection}
To identify the confounding tokens $A$ that introduce spurious correlations, we adopt a \textbf{gradient-based approach}~\citep{simonyan2013deep,sundararajan2017axiomatic} to quantitatively measure the influence of each token on the model's output $Y$. 
%=
Specifically, we leverage the gradient sensitivity of both the teacher model $\boldsymbol{\theta}_T$ and the student model $\boldsymbol{\theta}_S$. 
%=
We focus on data instances mispredicted by the student but correctly handled by the teacher to isolate confounding tokens.
%=
For each token $x_i \in X$, we compute the gradient of the loss with respect to that token for both models:
\begin{equation}
    g^{(T)}_i = \left| \frac{\partial \ell(x_i \mid X; \boldsymbol{\theta}_T)}{\partial x_i} \right|, 
    \quad 
    g^{(S)}_i = \left| \frac{\partial \ell(x_i \mid X; \boldsymbol{\theta}_S)}{\partial x_i} \right|.
\end{equation}
These gradients reflect the sensitivity of each model to perturbations in $x_i$.
%=
To enable token-level comparison between models with differing gradient scales, we apply min-max normalization to the sensitivity values.
\begin{equation}
    \hat{g}^{(T)}_i = \frac{g^{(T)}_i - \min_j g^{(T)}_j}{\max_j g^{(T)}_j - \min_j g^{(T)}_j}, 
    \quad 
    \hat{g}^{(S)}_i = \frac{g^{(S)}_i - \min_j g^{(S)}_j}{\max_j g^{(S)}_j - \min_j g^{(S)}_j}.
\end{equation}
To identify confounding tokens, we capture the difference in token-level attention between the teacher and student models by computing the gradient difference for each token:
\begin{equation}
    \Delta \hat{g}_i = \hat{g}^{(T)}_i - \hat{g}^{(S)}_i.
\end{equation}
% To ensure consistency in the scale of gradient differences across all samples, we normalize the gradient difference \( \Delta \hat{g}_i \) as follows:

% \begin{equation}
% \hat{\Delta \hat{g}}_i = \frac{\Delta \hat{g}_i - \min_j \Delta \hat{g}_j}{\max_j \Delta \hat{g}_j - \min_j \Delta \hat{g}_j}.
% \end{equation}
To ensure consistent scaling of gradient discrepancies across instances, we normalize the gradient difference and classify a token \( x_i \) as a \textbf{Confounding Token} if (i) it receives significant attention from the student model but negligible attention from the teacher during inference, as formalized in Equation~\ref{eq:confounder_threshold}, and (ii) its removal results in correct predictions from both models.
\begin{equation}
\label{eq:confounder_threshold}
\frac{\Delta \hat{g}_i - \min_j \Delta \hat{g}_j}{\max_j \Delta \hat{g}_j - \min_j \Delta \hat{g}_j} \leq \tau_{\text{confounder}},
\end{equation}
where \( \tau_{\text{confounder}} \) is a threshold determined via statistical analysis on a validation set. Sensitivity analyses on the threshold are presented in Section~\ref{apex:threshold}.
%=
Intuitively, confounding tokens capture sensitivity discrepancies between the teacher and student models that indicate spurious dependencies.
%=

Moreover, we also explored perplexity-based detection, but without teacher guidance, it tends to capture tokens indicative of model uncertainty rather than true confounders, especially on challenging tasks like the Olympiads. Accordingly, we adopt gradient-based detection as our primary strategy (see Section~\ref{sec:masking-analysis} for details).
% We also explored PPL-based methods for identifying confounding tokens.
% However, without supervision from a stronger teacher, PPL tends to capture tokens reflecting model uncertainty rather than true confounders (especially in complex task like Olympiad). accordingly, we adopt gradient-based detection as our primary strategy (see Section~\ref{sec:masking-analysis} for details).
% We also explored PPL-based methods for identifying confounding tokens.
% However, without supervision from a stronger teacher, PPL tends to capture internal confusion rather than true distracting patterns—especially on difficult datasets like Olympiad.
% Thus, we adopt the gradient-based approach as our main strategy (see Section~\ref{sec:masking-analysis} for details).

% \paragraph{Causal Attention Distillation} 

 
% \paragraph{Causal Attention Distillation}
\paragraph{Pruning Strategies.}
We study two pruning strategies for removing confounding tokens from instruction \(X\): (1) \textbf{Collective Pruning}, which removes the entire set of identified confounders \(A\), yielding \(X \setminus A\).
(2) \textbf{Span Pruning}, which removes only one contiguous confounding span \(A_i\) at a time, yielding \(X \setminus A_i\). 
%=
Preliminary experiments show that span pruning outperforms collective pruning (see Appendix \ref{apex:separate}), as pruning all distracting patterns simultaneously disrupts sentence integrity. Hence, we construct the augmented dataset via the span pruning strategy:
%=
\[
\mathcal{D}_{\mathrm{pruned}}
= \bigl\{(X \setminus A_i, y)\bigr\}_{i=1}^{k},
\]
where each \(A_i\) denotes a distinct confounding span. This augmentation encourages the model to learn reasoning paths invariant to specific confounders. 
\begin{figure}[t!]
    \centering
    \includegraphics[width=1\textwidth]{Figures/span_masking.pdf} % 修改路径为你的图片路径
    \caption{Illustration of Collective Pruning and Span Pruning.}
    \label{fig:span_masking}
    % \vspace{-0.7cm}
\end{figure}
\subsubsection{Causal Attention Distillation} 
\label{causal_attention}
After generating both original and counterfactual samples, we optimize two complementary distillation objectives to steer the student toward true causal dependencies:

\textbf{Standard Distillation.} align the student’s output distribution with the teacher’s on original instructions:
\[
\mathcal{L}_{kd} = D_{\mathrm{KL}}\bigl(p_T(y\mid X)\,\|\,p_S(y\mid X)\bigr),
\]
where $p_T$ and $p_S$ denote the teacher and student output distributions, respectively.

\textbf{Counterfactual Distillation.} align the student’s output distribution with the teacher’s on counterfactual instructions $X\setminus A$ (confounders pruned):
\[
\mathcal{L}_{cd} = D_{\mathrm{KL}}\bigl(p_T(y\mid X\setminus A)\,\|\,p_S(y\mid X\setminus A)\bigr).
\]
we blend these objectives with a weighting factor $\lambda$:
\[
\mathcal{L} = \lambda\,\mathcal{L}_{kd} \;+\; (1-\lambda)\,\mathcal{L}_{cd},
\]
where $\lambda\in[0,1]$ controls the trade-off between standard and counterfactual distillation. This composite loss steers the student to preserve semantic knowledge while enforcing genuine causal dependencies.

\paragraph{Response Splitting Strategies.} For our methods, we consider two variants: (1) \textbf{Instruct-level Pruning}: We detect and mask confounding tokens only in the instructions, and perform our LeaF on the instruction-level masked samples. (2) \textbf{Both Instruct- and Response-level Pruning}: We can also treat previously generated tokens as contextual input, and mask those that are misleading for subsequent generation, in order to help the model produce more accurate continuations. Thus, we detect and prune confounding tokens in both instructions and preceding generations.

\begin{figure}[htp]
    \centering
    \includegraphics[width=1\textwidth]{Figures/instruct_mislead_explain.pdf} % 修改路径为你的图片路径
    \caption{Illustration of Response Splitting Strategies: Language CoT, Instruct-level Pruning, and Response-level Pruning (2-segment and 3-segment splits). Highlighted white areas represent the input, and \textcolor{blue}{\underline{blue underlined areas}} represent the outputs used for cross-entropy loss computation.}
    \label{fig:instruct_cot_level_explain}
    % \vspace{-0.7cm}
\end{figure}


% preliminary experiments (Appendix~\ref{apex:separate}) show that span pruning outperforms collective pruning.

% \paragraph{Pruning Strategies:} 
% We compare two pruning strategies (Figure~\ref{fig:span_masking}): (1) \textbf{Collective Pruning}, which simultaneously masks all identified confounding tokens. (2) \textbf{Span Pruning}, which masks only contiguous spans of tokens.

% After identifying the confounding tokens $A$ (confounders) that induce spurious dependencies, we construct a pruned instruction representation $X_{\backslash A}$ by removing them from $X$. This operation effectively eliminates spurious paths from $A$ to $Y$ in the causal graph. 
% %=

% Preliminary experiments show that span pruning outperforms collective pruning (see Appendix \ref{apex:separate}), as masking all distracting patterns simultaneously disrupts sentence integrity. Hence, we generate multiple pruned perturbations via the span pruning strategy:
% \[
% \mathcal{D}_{\text{masked}} = \{(X_{\backslash A}, Y), (X_{\backslash A'}, Y), (X_{\backslash A''}, Y), \dots\}
% \]
% where $A', A''$ represent distinct distracting patterns within the instruction.  This augmentation encourages the model to learn reasoning paths invariant to specific confounders. 

%通过Preliminary experiments，我们发现span pruning achieves superior performance than collective pruning for the reason masking all distracting patterns disrupts sentence integrity, resulting in suboptimal training signals. Thus, we generate multiple pruned perturbations by span pruning strategy:
%=
% To better preserve semantic integrity, we treat continuous confounding tokens as complete distracting patterns. 
%=
% Preliminary experiments indicate that each misleading pattern separately, rather than collectively, achieves superior performance (see Appendix\ref{apex:separate} for details).
%= 
% We hypothesize that simultaneously masking all distracting patterns disrupts sentence integrity, resulting in suboptimal training signals. Thus, we generate multiple masked perturbations by separately masking each misleading pattern:
% To enhance robustness, we generate multiple perturbations of the masked tokens:

% where $\lambda \in [0, 1]$ balances the influence of standard and pruning-based distillation. This composite loss function drives the student model to learn both robust semantic dependencies and causal consistency. 
% \paragraph{Mixed Distillation Training with Causal Interventions} 
% To operationalize our causal intervention strategy, we integrate two types of samples for distillation: 
% \textbf{(1) Standard Knowledge Distillation Data}: These are conventional distillation samples where the student learns from the teacher's soft labels:
% \begin{equation}
%     \mathcal{L}_{KD} = D_{\text{KL}}(p_T(y \mid X) \parallel p_S(y \mid X)),
% \end{equation}
% where $p_T$ and $p_S$ denote the teacher and student output distributions, respectively. This standard knowledge distillation approach is widely adopted for improving smaller models' performance and thus serves as the baseline in our experiments.

% \textbf{(2) Counterfactual Distillation}: These are the samples generated by tokens pruning introduced above, where confounding tokens are removed from the instruction:
% \begin{equation}
%     \mathcal{L}_{LeaF} = D_{\text{KL}}(p_T(y \mid X_{\backslash A}) \parallel p_S(y \mid X_{\backslash A})).
% \end{equation}
% Here, $X_{\backslash A}$ reflects the counterfactual scenario where spurious dependencies are eliminated, allowing the student to learn purely causal paths.





==> hhcfmqnhvcmhjgxhytsngfvvpqzcbcgv/sections/03_method_new.tex <==
\section{Methodology}
\subsection{Causal Framework}

Following Pearl's Structural Causal Model~\cite{pearl2010causal}, we formulate a DAG $G$ to model the causal relationships among different components (refer to Figure~\ref{fig:causal_graph}). We assume the distribution of $(X, A, Y)$ is faithful to the DAG. In this framework,  \( X = [x_1, x_2, \dots, x_n] \) represents the input tokens, and $Y$ is the model's output. 
We define confounding tokens as a subset $A$ that obscure true causal relationships by introducing spurious correlations with both the output $Y$ and the complementary input $X \setminus A$. These misleading dependencies distort the model’s attention mechanisms and bias its reasoning process, ultimately yielding unreliable predictions.
 
% Confounding tokens, denoted as $A$, are a subset of $X$ that introduce spurious correlations during reasoning. Unlike regular tokens that convey semantic information, confounding tokens hide the true causal relationship, leading to incorrect predictions. 
% %=
% Spurious correlations between the subset $A$ and both the output $Y$ and the remaining input tokens $X \setminus A$ can mislead the model's attention allocation, resulting in biased and unreliable predictions.

% $A$ interfere with the output $Y$ by introducing erroneous correlations. This spurious dependency not only distorts the model's attention but also biases its output, leading to unreliable predictions.
% To better understand the DAG, we construct two hypotheses to describe the influence of confounding tokens $A$ on the generation process of $Y$:

\begin{wrapfigure}{r}{0.48\linewidth}
\vspace{-0.7cm}
    \centering
    \includegraphics[width=1\linewidth]{Figures/Causal_graph.pdf}
\setlength{\abovecaptionskip}{-0.8em}  
    \caption{Causal graph of the reasoning process. $X$ represents the input prompt, and $Y$ denotes the model's output. A subset of tokens in $X$, identified as confounding tokens ($A$), introduces spurious correlations that disrupt the reasoning process. Our method detects and masks $A$, effectively eliminating the spurious edge from $A$ to $Y$ and restoring the true causal dependency.}
    \label{fig:causal_graph}
    \vspace{-1.18cm}  
\end{wrapfigure}
% \paragraph{$\mathcal{H}_0$: There is no causal edge from $A$ to $Y$.}
% In this scenario, $A$ does not interfere with the generation of $Y$, and the model's reasoning path is purely determined by the meaningful tokens in $X \setminus A$. Formally, $A$ and $Y$ are \textbf{d-separated}
% given $X \setminus A$, 
% which implies:
% \begin{equation}
%     P(Y \mid X) = P(Y \mid X \setminus A).
% \end{equation}

% \paragraph{$\mathcal{H}_1$: There is a spurious correlation between $A$ to $Y$.}
% \paragraph{$\mathcal{H}_1$: There is a nonzero causal edge from \(A\) to \(Y\).}
% Equivalently, \(A\) and \(Y\) are not d-separated given \(X \setminus A\), which implies
% \[
% P(Y \mid X) \;\neq\; P\bigl(Y \mid X \setminus A\bigr).
% \]
% In this case, 

% \subsection{d-Separation and Causal Inference}
The desired behavior of the model is to \textbf{eliminate spurious correlations} introduced by confounding tokens $A$. When $A$ influences both $X$ and $Y$ (see dashed arrows in Figure~\ref{fig:causal_graph}), the observed conditional distribution becomes:
\begin{align}
    P &(Y \mid X_i = x) = \nonumber \\
    &\sum_{A} P(Y \mid X_i = x, A) \, P(A \mid X_i = x),
\end{align}
which deviates from the interventional distribution $P(Y \mid \text{do}(X_i))$ and reflects bias introduced by the indirect influence of $A$ on $Y$ through spurious paths.
% This discrepancy from the interventional distribution $P(Y \mid \text{do}(X_i))$ reflects the presence of active confounding paths, as $A$ and $Y$ are not d-separated by $X$ in the causal graph $G$.

To block these non-causal influences, we propose \textbf{causal pruning}, which removes the effect of $A$ prior to distillation. This encourages the student model to learn attention patterns grounded in true causal structure, improving robustness and interpretability.


\subsection{\texttt{LeaF}: Learning to Focus Framework}
\label{sec:LeaF}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\textwidth]{Figures/main_.pdf} % 修改路径为你的图片路径
    \caption{\textbf{Method Overview.} The training pipeline comprises two key stages: (1) \textbf{Confounding Token Detection}: gradient-based comparisons between an advanced teacher model and the student model are used to identify confounding tokens in the training samples and constructs counterfactual samples by pruning these tokens; and (2) \textbf{Causal Attention Distillation}: prune identified confounders respectively during training to align the student’s attention with the teacher’s and capture casual relationships. This targeted intervention steers the model toward actual causal dependencies, enhancing both robustness and interpretability.}
    \label{fig:main}
    \vspace{-0.3cm}
\end{figure}

% To achieve the desired d-separation and eliminate spurious dependencies, we introduce a \textbf{Learning to Focus Framework (LeaF)} (Figure ~\ref{fig:main}), which consists of two main stages:  
% (1) Confounding Token Detection (Section~\ref{misleading_tokens_detection}) and (2) Causal Attention Distillation (Section~\ref{causal_attention}). We discuss them in detail in the following.
To eliminate spurious dependencies, we introduce the \textbf{Learning to Focus (LeaF)} framework (Figure ~\ref{fig:main}), which consists of two main stages:  
(1) Confounding Token Detection (Section~\ref{misleading_tokens_detection}), where LeaF identifies confounding tokens via teacher–student gradient-based comparisons and constructs counterfactual samples by pruning these tokens.
(2) Causal Attention Distillation (Section~\ref{causal_attention}), where LeaF captures causal dependencies through a hybrid distillation loss that aligns the student with the teacher on both original and counterfactual samples.
We discuss them in detail in the following.
\subsubsection{Confounding Token Detection} \label{misleading_tokens_detection}
To identify the confounding tokens $A$ that introduce spurious correlations, we adopt a \textbf{gradient-based approach}~\citep{simonyan2013deep,sundararajan2017axiomatic} to quantitatively measure the influence of each token on the model's output $Y$. 
%=
Specifically, we leverage the gradient sensitivity of both the teacher model $\boldsymbol{\theta}_T$ and the student model $\boldsymbol{\theta}_S$. 
%=
We focus on data instances mispredicted by the student but correctly handled by the teacher to isolate confounding tokens.
%=
% For each token $x_i \in X$, we compute the gradient of the loss with respect to that token for both models:
For each token $x_i \in X$, we compute the gradient of the cross-entropy loss between predicted logits and gold references with respect to the embedding of $x_i$ for both models.
\begin{equation}
    g^{(T)}_i = \left| \frac{\partial \ell(x_i \mid X; \boldsymbol{\theta}_T)}{\partial x_i} \right|, 
    \quad 
    g^{(S)}_i = \left| \frac{\partial \ell(x_i \mid X; \boldsymbol{\theta}_S)}{\partial x_i} \right|.
\end{equation}
These gradients reflect the sensitivity of each model to perturbations in $x_i$.
%=
To enable token-level comparison between models with differing gradient scales, we apply min-max normalization to the sensitivity values.
\begin{equation}
    \hat{g}^{(T)}_i = \frac{g^{(T)}_i - \min_j g^{(T)}_j}{\max_j g^{(T)}_j - \min_j g^{(T)}_j}, 
    \quad 
    \hat{g}^{(S)}_i = \frac{g^{(S)}_i - \min_j g^{(S)}_j}{\max_j g^{(S)}_j - \min_j g^{(S)}_j}.
\end{equation}
To identify confounding tokens, we capture the difference in token-level attention between the teacher and student models by computing the gradient difference for each token:
\begin{equation}
    \Delta \hat{g}_i = \hat{g}^{(T)}_i - \hat{g}^{(S)}_i.
\end{equation}

To ensure consistent scaling of gradient discrepancies across instances, we normalize the gradient difference and classify a token \( x_i \) as a \textbf{Confounding Token} if (i) it receives significant attention from the student model but negligible attention from the teacher during inference, as formalized in Equation~\ref{eq:confounder_threshold}, and (ii) its removal results in correct predictions from both models.
\begin{equation}
\label{eq:confounder_threshold}
\frac{\Delta \hat{g}_i - \min_j \Delta \hat{g}_j}{\max_j \Delta \hat{g}_j - \min_j \Delta \hat{g}_j} \leq \tau_{\text{confounder}},
\end{equation}
where \( \tau_{\text{confounder}} \) is a threshold determined via statistical analysis on a validation set. Sensitivity analyses on the threshold are presented in Section~\ref{apex:threshold}.
%=
Intuitively, confounding tokens capture sensitivity discrepancies between the teacher and student models that indicate spurious dependencies.
%=

Moreover, we also explored perplexity-based detection, but without teacher guidance, it tends to capture tokens indicative of model uncertainty rather than true confounders, especially on challenging tasks like the Olympiads. Accordingly, we adopt gradient-based detection as our primary strategy (see Section~\ref{sec:masking-analysis} for details).

\paragraph{Pruning Strategies.}
We study two pruning strategies for removing confounding tokens from instruction \(X\): (1) \textbf{Collective Pruning}, which removes the entire set of identified confounders \(A\), yielding \(X \setminus A\).
(2) \textbf{Span Pruning}, which removes only one contiguous confounding span \(A_i\) at a time, yielding \(X \setminus A_i\). 
%=
Preliminary experiments show that span pruning outperforms collective pruning (see Appendix \ref{apex:separate}), as pruning all distracting patterns simultaneously disrupts sentence integrity. Hence, we construct the counterfactual samples via the span pruning strategy:
%=
\[
\mathcal{D}_{\mathrm{pruned}}
= \bigl\{(X \setminus A_i, y)\bigr\}_{i=1}^{k},
\]
where each \(A_i\) denotes a distinct confounding span. This augmentation encourages the model to learn reasoning paths invariant to specific confounders. 
\begin{figure}[t!]
    \centering
    \includegraphics[width=1\textwidth]{Figures/span_masking.pdf} % 修改路径为你的图片路径
    \caption{Illustration of Collective Pruning and Span Pruning.}
    \label{fig:span_masking}
    % \vspace{-0.7cm}
\end{figure}
\subsubsection{Causal Attention Distillation} 
\label{causal_attention}
After generating both original and counterfactual samples, we optimize two complementary distillation objectives to steer the student toward true causal dependencies:

\textbf{Standard Distillation.} Align the student’s output distribution with the teacher’s on original instructions:
\[
\mathcal{L}_{kd} = D_{\mathrm{KL}}\bigl(p_T(y\mid X)\,\|\,p_S(y\mid X)\bigr),
\]
where $p_T$ and $p_S$ denote the teacher and student output distributions, respectively.

\textbf{Counterfactual Distillation.} Align the student’s output distribution with the teacher’s on counterfactual instructions $X\setminus A$ (confounders pruned):
\[
\mathcal{L}_{cd} = D_{\mathrm{KL}}\bigl(p_T(y\mid X\setminus A)\,\|\,p_S(y\mid X\setminus A)\bigr).
\]
we blend these objectives with a weighting factor $\lambda$:
\[
\mathcal{L} = \lambda\,\mathcal{L}_{kd} \;+\; (1-\lambda)\,\mathcal{L}_{cd},
\]
where $\lambda\in[0,1]$ controls the trade-off between standard and counterfactual distillation. This composite loss steers the student to preserve semantic knowledge while enforcing genuine causal dependencies.

\paragraph{Response Splitting Strategies.} For our methods, we consider two variants: (1) \textbf{Instruct-level Pruning}: We detect and prune confounding tokens only in the instructions, and perform our LeaF on the instruction-level pruned samples. (2) \textbf{Both Instruct- and Response-level Pruning}: We can also treat previously generated tokens as contextual input, and prune those that are misleading for subsequent generation, in order to help the model produce more accurate continuations. Thus, we detect and prune confounding tokens in both instructions and preceding generations.

\begin{figure}[htp]
    \centering
    \includegraphics[width=1\textwidth]{Figures/instruct_mislead_explain.pdf} % 修改路径为你的图片路径
    \caption{Illustration of Response Splitting Strategies: Language CoT, Instruct-level Pruning, and Response-level Pruning (2-segment and 3-segment splits). Highlighted white areas represent the input, and \textcolor{blue}{\underline{blue underlined areas}} represent the outputs used for cross-entropy loss computation.}
    \label{fig:instruct_cot_level_explain}
    % \vspace{-0.7cm}
\end{figure}




==> hhcfmqnhvcmhjgxhytsngfvvpqzcbcgv/sections/04_results.tex <==
\section{Experiments}

% We conduct experiments in both mathematical reasoning and code generation domains to explore the effectiveness of our proposed method LeaF.

\subsection{Experiment Settings}

% We conduct experiments to evaluate the effectiveness of Learning to Focus Framework (LeaF) on both mathematical reasoning and code generation tasks. We perform comprehensive evaluations on standard benchmarks to assess improvements in consistency, accuracy, and robustness.  

\textbf{Training Datasets.} We conduct experiments to evaluate the effectiveness of our proposed method Learning to Focus Framework (LeaF) on mathematical reasoning, code generation, and multi-hop question answering tasks.
%=
For mathematical reasoning, to ensure the model encounters an equal number of confounding tokens across tasks, we randomly select 30k instances from each of the following subsets in NuminaMath-CoT~\cite{numina_math_datasets}: Olympiads~\cite{he2024olympiadbench}, AMC$\_$AIME~\cite{numina_math_datasets}, GSM8K~\cite{cobbe2021gsm8k}, and MATH~\cite{math_benchmark}.
For code generation, we randomly select a subset of 120k instances from the AceCode-87k~\cite{AceCoder} dataset.
%=
For multi-hop question answering, we construct the training set by merging the KILT~\cite{petroni2020kilt} datasets provided in Helmet~\cite{yen2024helmet}, totaling 3k annotated samples drawn equally from HotpotQA~\cite{yang2018hotpotqa}, NQ~\cite{nq2021}, and PopQA~\cite{popqa2022}, where each query is explicitly linked to its corresponding gold passages containing the answers.
% 这里具体介绍训练时候数据集的构成
% For mathematical reasoning, we utilize four major datasets: GSM8K, MATH, Olympiad, and AIME. We curated a total of 12,000 high-quality mathematical problems with balanced distribution across these datasets (3,000 samples each). For code generation, we collect samples from the Magicode OSS and Magicode Evol datasets, summing up to 12,000 code-related problems (6,000 samples each). These datasets are designed to cover a broad spectrum of problem types and difficulty levels, providing a diverse pretraining foundation for LeaF. 

\textbf{Evaluation Datasets.}
For math task evaluation, we select three widely used benchmarks with varying levels of difficulties, including GSM8K~\cite{cobbe2021gsm8k}, MATH-500~\cite{math_benchmark}, and OlympiadBench~\cite{he2024olympiadbench}. In code domain, we conduct evaluations on HumanEval+\cite{evalplus}, LeetCode\cite{leetcode}, and LivecodeBench (v4)\cite{jain2024livecodebench}, providing a comprehensive assessment across diverse aspects of coding performance. For multi-hop question answering, we evaluate on three representative benchmarks, including HotpotQA~\cite{yang2018hotpotqa}, 2WikiMultiHopQA~\cite{ho2020constructing}, and Musique~\cite{trivedi2022musique}.
The detailed description of the mathematical reasoning, code generation and multi-hop QA benchmarks is provided in Appendix~\ref{apex: benchmark}.

% For mathematical problem solving, we evaluate our model on tasks of varying difficulty: spanning school-level, university-level, and competition-level, using the GSM8K, Math, and Olympiad benchmarks. 
%We apply uniform sampling settings to ensure consistency across models during inference: temperature = 0.0 and top_p = 1.0 for all math benchmarks. For code generation, we assess model performance on HumanEval(+), Leetcode, and LiveCodeBench, using pass@1 for HumanEval(+) and Leetcode, and pass@10 for LiveCodeBench.

\textbf{Base Models and Baselines.} 
We conduct comprehensive experiments on two different model families, LLaMA family~\citep{llama,liu2024llama3b} and Qwen family~\cite{yang2024qwen2}, covering various sizes of models. For LLaMA-based experiments, we employ LLaMA3.2-1B-Instruct~\cite{liu2024llama3b} and LLaMA3.2-3B-Instruct~\cite{liu2024llama3b} as student models, while their teacher models are set as LLaMA3.3-70B-Instruct~\cite{liu2024llama3b}. For Qwen-based experiments, we use Qwen2.5-Math-1.5~\cite{yang2024qwen2} as the student model, with Qwen2.5-72B-Instruct~\cite{yang2024qwen2} as the teacher model.
Our baseline for comparison is standard knowledge distillation without pruning. We use the CoT-based variant for math and the vanilla variant for code generation and multi-hop QA.
% Our baseline for comparison is the standard knowledge distillation method, which involves no pruning procedure. CoT-based for math tasks and vanilla for code and QA.
% We employ LLaMA 3.2 1B and 3B Instruct as student models, while their teacher models are set as LLaMA 3.3 70B Instruct. For Qwen-based experiments, we use Qwen 2.5-math-1.5 as the student model, with Qwen 2.5 72B as the teacher model. Training is performed on 64 A100 GPUs with a batch size of 1M tokens per step. The maximum sequence length is set to 2048 tokens for 1B models and 4096 tokens for 3B models, applying a cosine decay learning rate scheduler. All models are trained for 3 epochs, with an initial learning rate of $5e^{-5}$ for 1B models and $1e^{-5}$ for 3B models.  

\begin{table*}[t!]
\caption{Performance on MathBench and CodeBench for Instruct models (LLaMA 3.2–1B/3B-Instruct) and Base model (Qwen 2.5–Math-1.5B) under three pruning schemes (no mask, Instruct-level Mask, and Response-level Mask), where Instr Mask refers to Instruct-level pruning, and Resp Mask refers to Response-level pruning. The best and second-best results are marked in \textbf{bold} and \underline{underlined}, respectively.}
\label{tab: main results}
\vskip 0.1in
\centering
\small
\setlength{\tabcolsep}{3.25pt}
% \sisetup{detect-all,mode=text}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccccccc} 
\toprule
\multicolumn{1}{c}{\multirow[b]{2}{*}{Model}}
  & \multicolumn{4}{c}{MathBench}
  & \multicolumn{4}{c}{CodeBench} \\
\cmidrule(lr){2-5}
\cmidrule(lr){6-9}
  & GSM8K
  & MATH-500
  & \begin{tabular}[c]{@{}c@{}}Olympiad-\\Bench\end{tabular}
  & Avg.
  & \begin{tabular}[c]{@{}c@{}}Human-\\Eval+\end{tabular}
  & \begin{tabular}[c]{@{}c@{}}Leet-\\Code\end{tabular}
  & \begin{tabular}[c]{@{}c@{}}Livecode-\\Bench\end{tabular}
  & Avg. \\
\midrule
\multicolumn{9}{l}
{\emph{\quad \textbf{Teacher Model}}} \\
LLaMA3.3-70B-Instruct & 95.60 & 70.40 & 36.50 &67.50 & 78.05&53.90 &45.02 & 58.99 \\
Qwen2.5-72B-Instruct & 95.45 & 73.80 & 41.25 & 70.17 &81.71 &69.40 & 54.42 & 68.51 \\
\midrule
\multicolumn{9}{l}
{\emph{\quad \textbf{LLaMA3.2-1B-Instruct}}} \\
Instruct Model (Pre-KD) & 44.88 & 24.20 & 5.79& 24.96  & 29.27 & \textbf{7.22} & 9.68& 15.39 \\
% SFT w/o Mask & 48.90 & 31.60 & 6.23 & 28.91 & 37.80& 1.11&0.00 & 12.60 \\
KD w/o Mask & 56.79 & 33.40 & 8.90 & 33.03  & 32.32 & 6.11 & \textbf{13.74} & 17.39 \\
LeaF (Instr Mask)  & \underline{57.70} & \textbf{35.40} & \textbf{10.09} & \underline{34.40} & 39.02  & \underline{6.67} & \underline{13.60} & \underline{19.76} \\
LeaF (Instr \& Resp Mask) & \textbf{58.98} & \underline{35.20} & \underline{9.94} &\textbf{34.71} & \textbf{39.63} & \textbf{7.22} & 12.48& \textbf{19.77} \\
\midrule
\multicolumn{9}{l}{\emph{\quad \textbf{LLaMA3.2-3B-Instruct}}} \\
Instruct Model (Pre-KD) & 76.88 & 42.80 &13.20 & 44.29 & 48.78 & 13.89 & 20.34 & 27.67 \\
% SFT w/o Mask & 80.21 & 47.40 & 17.51 &48.37 & \textbf{58.54}&4.40 & 3.51& 15.12 \\
KD w/o Mask &  82.87&49.00&18.99&50.29& 54.88 & 16.67 & 24.12 & 31.89\\
LeaF (Instr Mask) &  \underline{83.09} & \underline{51.80} & \underline{20.77} & \underline{51.88} & 55.49 & \underline{19.44}  & \underline{25.39}& \underline{33.44} \\
LeaF (Instr \& Resp Mask) & \textbf{84.69} & \textbf{52.40} & \textbf{22.55} & \textbf{53.21} & \underline{56.10} & \textbf{21.67} &\textbf{25.81} & \textbf{34.53} \\
\midrule
\multicolumn{9}{l}{\emph{\quad \textbf{Qwen2.5-Math-1.5B}}} \\
Base Model (Pre-KD) & 65.20 & 41.40 & 21.96& 42.85 & 35.37 & 6.67 & 1.26 & 14.43\\
% SFT w/o Mask & \underline{85.06} & 65.40 & 31.16& 60.54& \textbf{55.49}&0.00 &0.00 & 18.50 \\
KD w/o Mask & 82.18 & 67.80 & 31.16 & 60.38  & 41.46& \underline{7.78} & 10.10 & 19.78\\
LeaF (Instr Mask) & 84.69 & \underline{68.60} & \textbf{32.79} & \underline{62.03} & 42.68 & \textbf{9.94} & \underline{10.80} & \underline{20.97}\\
LeaF (Instr \& Resp Mask) & \textbf{85.29} & \textbf{70.60} & \underline{31.75} & \textbf{62.54}  & \underline{43.29}  & \textbf{9.94} & \textbf{13.04}& \textbf{21.92} \\
\bottomrule
\end{tabular}
\end{adjustbox}
% \begin{tablenotes}[flushleft]
%   \scriptsize
%   \item[1] \textbf{KD w/o Mask:} standard knowledge distillation without any masking.  
%   \item[2] \textbf{LeaF (Instr Mask):} distillation with instruction-level misleading-token masking.  
%   \item[3] \textbf{KD + Instr \& CoT Mask:} distillation with both instruction- and chain-of-thought misleading-token masking.
% \end{tablenotes}
% \vspace{-0.5cm}
\end{table*}

\begin{table*}[t!]
\caption{Performance on multi-hop QA benchmarks under different pruning strategies. Given the short response length of multi-hop QA tasks, only the LeaF (Instruct-level Mask) variant is evaluated. Given the long-context requirement of multi-hop QA, we validate LeaF using LLaMA-3.2-3B-Instruct.}
\label{tab:multihop_results}
\vskip 0.1in
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lccccccccc c} 
\toprule
\multirow{2}{*}{Model} 
& \multicolumn{3}{c}{2WikiMultiHopQA} 
& \multicolumn{3}{c}{Musique} 
& \multicolumn{3}{c}{HotpotQA} 
& \multirow{2}{*}{Avg.} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
& EM & F1 & SubEM 
& EM & F1 & SubEM 
& EM & F1 & SubEM 
&  \\
\midrule
\multicolumn{9}{l}{\emph{\quad \textbf{LLaMA3.2-3B-Instruct}}} \\
Instruct Model (Pre-KD) & 22.50 & 34.73 & 45.50 & 9.50 & 16.56 & 18.50 & 19.50 & 32.67 & 36.00 & 26.16 \\
KD w/o Mask & \underline{43.50} & \underline{51.93} & \underline{53.00} & \underline{20.50} & \underline{28.56} & \underline{22.50} & \underline{39.00} & \underline{49.30} & \underline{43.00} & \underline{39.03} \\
LeaF (Instr Mask)  & \textbf{46.50} & \textbf{53.89} & \textbf{55.00} & \textbf{27.00} & \textbf{33.00} &  \textbf{28.00} & \textbf{40.50} & \textbf{52.06} & \textbf{44.50} & \textbf{42.27} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

% \textbf{Baselines} 
%  Our baseline for comparison is the naive knowledge distillation method, which involves no pruning procedure.


%We compare our method against standard knowledge distillation and carry out ablation studies to quantify the effect of each component: (1) Distillation without any masking, (2) Distillation with only instruction‐level misleading‐token masking, and (3) Distillation with both instruction- and chain-of-thought misleading-token masking. The detailed results are discussed in Section 4.

\textbf{Training and Evaluation Settings.} 
%放training 和evaluation 的设定，例如hyper-parameters
(1) During training, models are trained using the Alpaca-LoRA framework with full-parameter logits knowledge distillation and a cosine learning rate schedule with a maximum learning rate of $10^{-5}$ for three epochs. The batch size is 64 for LLaMA-based models and 32 for Qwen-based models. Detailed hyperparameters and platform information are in Appendix~\ref{apex:training_detail}. (2) In evaluation, teacher and student models are evaluated on math, code and QA tasks using greedy decoding. The maximum generation length is 1024 tokens for code and 16,384 tokens for math tasks. Official chat templates are followed during inference. Full evaluation details are in Appendix~\ref{apex:evaluate_detail}.
%=

% We apply uniform sampling settings to ensure consistency across models during inference: temperature = 0.0 and top\_p = 1.0 for all math benchmarks. For code generation, we assess model performance on HumanEval(+), Leetcode, and LiveCodeBench, using pass@1 for HumanEval(+) and Leetcode, and pass@10 for LiveCodeBench.
% To evaluate our models, we use a range of benchmarks covering both mathematical reasoning and code generation:  
% - For math reasoning: GSM8K, MATH-500, Olympiad.  
% - For code generation: HumanEval+, Leetcode, and LiveCodeBench.  

% We utilize the llm-eval-harness~\cite{Gao2023} for general evaluation, and a custom evaluation suite for math-specific tasks. For efficient inference, we employ vllm (v0.3.2)~\cite{Kwon2023}. Further details about evaluation protocols can be found in Appendix A.  


% \textbf{Datasets.} 
% We conduct experiments on two datasets: a mathematical reasoning dataset consisting of \textbf{X} samples and a long-text comprehension dataset with \textbf{Y} samples. The datasets are preprocessed by tokenizing, cleaning, and splitting into training (70\%), validation (15\%), and test (15\%) sets.

% \textbf{Model Configurations.} 
% The teacher model is a pre-trained LLaMA-70B, and the student model is based on a Transformer architecture with \textbf{Z} parameters. Both models are fine-tuned on the same input instructions. The hyperparameters used in training are as follows: learning rate \(1 \times 10^{-4}\), batch size of 32, and a distillation weight \(\lambda\) set between 0.5 and 0.7. The thresholds for token selection are set to \(\tau_{imp}=0.6\) and \(\tau_{mis}=-0.2\).

% \textbf{Experimental Environment.} 
% All experiments are run on NVIDIA Tesla V100 GPUs using PyTorch 1.9 and Python 3.8. The full code is available at \url{https://github.com/xxx/xxx} for reproducibility.

% \textbf{Evaluation Metrics.} 
% For the mathematical reasoning task, we evaluate the models using accuracy and inference error rate. For the long-text comprehension task, ROUGE-1 and ROUGE-L scores are reported. Additionally, we perform qualitative analysis by visualizing the gradient distributions and attention heatmaps to illustrate the impact of the masking strategies.


% \subsection{Baselines and ablation studies.} 
% We compare our method against standard knowledge distillation and carry out ablation studies to quantify the effect of each component: (1) Distillation without any masking, (2) Distillation with only instruction‐level misleading‐token masking, and (3) Distillation with both instruction- and chain-of-thought misleading-token masking. The detailed results are discussed in Section 4.

\subsection{Main Results}
\label{sec:main_result}
% In this section, we compare the best performances of LeaF against baselines to assess how it benefits open-source LLMs. We evaluate the effectiveness of CPO across two evaluation tasks: MathBench (i.e., GSM8K, MATH, and Olympiad) and CodeBench (i.e., HumanEval+, Leetcode, and LivecodeBench).
% \paragraph{Evaluation Setting}
% (1) Open-source instruct models and base models. We select several publicly available aligned open-source models, including Llama-3.2-1B-Instruct, Llama-3.2-2B-Instruct, and Qwen2.5-Math-1.5B. The download links for these models are provided in Appendix~\ref{apex: opensource}.
% (2) LLMs trained via knowledge distillation. We also include LLMs that are trained using the same base model and training corpus via knowledge distillation.

% \paragraph{Results}
The main results are presented in Table~\ref{tab: main results} and Table~\ref{tab:multihop_results}. We can draw several conclusions from the results:
(1) For open-source baselines, both standard distillation and our approach lead to improvements in the performance of models across nearly all tasks in math, code and multi-hop
question answering domains.
(2) In terms of performance, LeaF consistently outperforms standard knowledge distillation when using the same training corpus. This suggests that LeaF has the potential to enable the model to attend to critical information more effectively, thereby enhancing its reasoning capabilities. 
(3) Extending from instruction-level to response-level pruning yields further performance improvements across most tasks in the LLaMA and Qwen series, suggesting that distracting patterns at the response level affect subsequent generations. We hypothesize that instruction-level and response-level distracting patterns differ, and simultaneously learning both can enhance the model's reasoning capabilities. A more detailed analysis based on the response splitting strategy is provided in Section~\ref{sec: response_split_strategy}. Additionally, Appendix~\ref{app:robustness} shows that LeaF is more robust than other pruning strategies.


% \begin{table*}[t]
% \caption{miao}
% \label{tab: main results1}
% \centering
% \small
% \setlength{\tabcolsep}{3.25pt}
% % \sisetup{detect-all,mode=text}
% \begin{adjustbox}{max width=\textwidth}
% \begin{tabular}{lcccccccc} 
% \toprule
% \multirow{2}{*}{Model}
%   & \multicolumn{4}{c}{ProcessBench}
%   & \multicolumn{4}{c}{CodeBench} \\
% \cmidrule(lr){2-5}
% \cmidrule(lr){6-9}
%   & GSM8K
%   & MATH
%   & \begin{tabular}[c]{@{}c@{}}Olympiad-\\Bench\end{tabular}
%   & Avg.
%   & \begin{tabular}[c]{@{}c@{}}Human-\\Eval+\end{tabular}
%   & \begin{tabular}[c]{@{}c@{}}Leet-\\code\end{tabular}
%   & \begin{tabular}[c]{@{}c@{}}Livecode-\\Bench\end{tabular}
%   & Avg. \\
% \midrule
% \multicolumn{9}{l}{\emph{\quad \textbf{Baseline Models}}} \\
% LLaMA3.2-1B-Instruct & 56.79 & 33.40 & 8.90 & 33.03  &  &  & & \\
% LLaMA3.2-3B-Instruct &  &  & &   &  &  & & \\
% Qwen2.5-Math-1.5B &  &  & &   &  &  & & \\
% Qwen2.5-1.5B-Instruct &  &  & &   &  &  & & \\
% \midrule
% \multicolumn{9}{l}{\emph{\quad \textbf{Stage 1: instruction only}}} \\
% LLaMA3.2-1B-Instruct &  &  & &   &  &  & & \\
% LLaMA3.2-3B-Instruct &  &  & &   &  &  & & \\
% Qwen2.5-Math-1.5B &  &  & &   &  &  & & \\
% Qwen2.5-1.5B-Instruct &  &  & &   &  &  & & \\
% \midrule
% \multicolumn{9}{l}{\emph{\quad \textbf{Stage 2: instruction and cot level}}} \\
% LLaMA3.2-1B-Instruct &  &  & &   &  &  & & \\
% LLaMA3.2-3B-Instruct &  &  & &   &  &  & & \\
% Qwen2.5-Math-1.5B &  &  & &   &  &  & & \\
% Qwen2.5-1.5B-Instruct &  &  & &   &  &  & & \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% % \vskip -0.1in
% \end{table*}


% \begin{table*}[htpb]
% \caption{Performance on MathBench and CodeBench for Instruct models (LLaMA 3.2–1B/3B-Instruct) and Base model (Qwen 2.5–Math-1.5B) under three masking schemes (no mask, Instruct-level Mask, and Response-level Mask), where Instr Mask refers to Instruct-level masking, and Resp Mask refers to Response-level masking. The best and second-best results are marked in \textbf{bold} and \underline{underlined}, respectively.}
% \label{tab: main results}
% \vskip 0.1in
% \centering
% \small
% \setlength{\tabcolsep}{3.25pt}
% % \sisetup{detect-all,mode=text}
% \begin{adjustbox}{max width=\textwidth}
% \begin{tabular}{lcccccccc} 
% \toprule
% \multicolumn{1}{c}{\multirow[b]{2}{*}{Model}}
%   & \multicolumn{4}{c}{MathBench}
%   & \multicolumn{4}{c}{CodeBench} \\
% \cmidrule(lr){2-5}
% \cmidrule(lr){6-9}
%   & GSM8K
%   & MATH
%   & \begin{tabular}[c]{@{}c@{}}Olympiad-\\Bench\end{tabular}
%   & Avg.
%   & \begin{tabular}[c]{@{}c@{}}Human-\\Eval+\end{tabular}
%   & \begin{tabular}[c]{@{}c@{}}Leet-\\Code\end{tabular}
%   & \begin{tabular}[c]{@{}c@{}}Livecode-\\Bench\end{tabular}
%   & Avg. \\
% \midrule
% \multicolumn{9}{l}{\emph{\quad \textbf{LLaMA3.2-1B-Instruct}}} \\
% Instruct Model (Pre-KD) & 44.88 & 24.20 & 5.79& 24.96  & 29.27 & \textbf{7.22} & 9.68& 15.39 \\
% KD w/o Mask & 56.79 & 33.40 & 8.90 & 33.03  & 32.32 & 6.11 & 13.74 & 17.39 \\
% LeaF (Instr Mask)  & \underline{57.70} & \textbf{35.40} & \textbf{10.09} & \underline{34.40} & 39.02  & \underline{6.67} & 13.60 & 19.76 \\
% LeaF (Instr \& Resp Mask) & \textbf{58.98} & \underline{35.20} & \underline{9.94} &\textbf{34.71} & \textbf{39.63} & \textbf{7.22} & 12.48& 19.77 \\
% \midrule
% \multicolumn{9}{l}{\emph{\quad \textbf{LLaMA3.2-3B-Instruct}}} \\
% Instruct Model (Pre-KD) & 76.88 & 42.80 &13.20 & 44.29 & 48.78 & 13.89 & 20.34 & 27.67 \\
% KD w/o Mask &  82.87&49.00&18.99&50.29& 54.88 & 16.67 & 24.12 & 31.89\\
% LeaF (Instr Mask) &  \underline{83.09} & \underline{51.80} & \underline{20.77} & \underline{51.88} & \underline{55.49} & \underline{19.44}  & \underline{25.39}& \underline{33.44} \\
% LeaF (Instr \& Resp Mask) & \textbf{84.69} & \textbf{52.40} & \textbf{22.55} & \textbf{53.21} & \textbf{56.10} & \textbf{21.67} &\textbf{25.81} & \textbf{34.53} \\
% \midrule
% \multicolumn{9}{l}{\emph{\quad \textbf{Qwen2.5-Math-1.5B}}} \\
% Base Model (Pre-KD) & 65.20 & 41.40 & 21.96& 42.85 & 35.37 & 6.67 & 1.26 & 14.43\\
% KD w/o Mask & 82.18 & 67.80 & 31.16 & 60.38  & 41.46& 7.78 & 10.10 & 19.78\\
% LeaF (Instr Mask) & \underline{84.69} & \underline{68.60} & \textbf{32.79} & \underline{62.03} & 42.68 & 9.94 & 10.80 & 20.97\\
% LeaF (Instr \& Resp Mask) & \textbf{85.29} & \textbf{70.60} & \underline{31.75} & \textbf{62.54}  &  &  & & \\
% % \midrule
% % \multicolumn{9}{l}{\emph{\quad \textbf{Qwen2.5-1.5B-Instruct}}} \\
% % Instruct Model (Pre-KD) & x & x & x& x  & 56.10 & 17.22 & 20.62 & 29.48\\
% % KD w/o Mask & 75.36 & 51.40 & 19.29 & 48.68 & 56.10 & 18.33 & 23.14& 32.52 \\
% % LeaF (Instr Mask) &  &  & &   &  &  & & \\
% % KD + Instr \& CoT Mask &  &  & &   &  &  & & \\
% % \midrule
% % \multicolumn{9}{l}{\emph{\quad \textbf{Qwen2.5-3B-Instruct}}} \\
% % % Instruct Model (Pre-KD) & x & x &x &  x & 68.90  & 32.22 & 25.67 & 42.26 \\
% % KD w/o Mask & 84.00 & 62.20 & 24.04 & 56.75  & 68.90 & 32.22 & 28.75 & 43.09\\
% % LeaF (Instr Mask) &  &  & &   &  &  & & \\
% % KD + Instr \& CoT Mask &  &  & &   &  &  & & \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% % \begin{tablenotes}[flushleft]
% %   \scriptsize
% %   \item[1] \textbf{KD w/o Mask:} standard knowledge distillation without any pruning.  
% %   \item[2] \textbf{LeaF (Instr Mask):} distillation with instruction-level misleading-token pruning.  
% %   \item[3] \textbf{KD + Instr \& CoT Mask:} distillation with both instruction- and chain-of-thought misleading-token pruning.
% % \end{tablenotes}
% \end{table*}

==> hhcfmqnhvcmhjgxhytsngfvvpqzcbcgv/sections/05_analysis.tex <==
\section{Further Analysis}
In this section, we conduct masking strategies analysis (Section~\ref{sec:masking-analysis}), response splitting analysis
(Section~\ref{sec: response_split_strategy}) and threshold sensitivity analysis~\ref{apex:threshold}. Finally, we present a case study (Section~\ref{sec:case_study}) to illustrate the interpretability of our approach. 
% Additional analyses on computational overhead and ablation studies are provided in Appendix~\ref{app:overhead} and Appendix~\ref{app:ablation}, respectively.
In the appendix, we include robustness analysis (Appendix~\ref{app:robustness}), threshold stability across tasks (Appendix~\ref{app:threshold}), computational overhead analysis (Appendix~\ref{app:overhead}), ablation study (Appendix~\ref{app:ablation}), and dataset statistics of counterfactual and original samples (Appendix~\ref{app:cf_stats}).

\subsection{Masking Strategies Analysis}
\label{sec:masking-analysis}


To demonstrate the effectiveness of our gradient-based masking strategy, we compare LeaF with two other choices of token masking: (1) \textbf{Random Masking}, where the same number of tokens identified by our gradient-based method are randomly masked for each instance; and (2) \textbf{PPL-based Masking}, where tokens with the highest perplexity scores are masked at the same ratio, following the same data filtering process used in our method to generate augmented training data. We evaluate all three masking strategies, Random Masking, PPL-based Masking, and Gradient-based Masking, on the GSM8K, MATH-500, and OlympiadBench datasets.

\paragraph{Results.} 
We present the results in Figure~\ref{fig:masking_strategy}. Our observations are as follows: (1) Gradient-based Masking (ours) consistently outperforms both baselines, with the highest accuracy on MATH-500 and OlympiadBench. (2) Random Masking leads to performance degradation on GSM8K and Olympiad, despite showing a slight improvement on MATH-500. This suggests that naively masking tokens without informed selection can undermine distillation performance. (3) PPL-based masking provides modest improvements on GSM8K and MATH-500, but performs comparably to random masking on OlympiadBench, indicating its limitations on complex tasks. Our analysis is, while perplexity may suffice for detecting confounding tokens in simpler settings, it lacks the sensitivity needed for challenging benchmarks. This highlights the necessity of an advanced teacher model to guide token selection in complex reasoning scenarios.
% \begin{table}[t]
% \caption{Performance comparison of different masking strategies on math benchmarks.}
% \label{tab:masking_strategies}
% \centering
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Masking Method}  & \textbf{GSM8K} & \textbf{MATH} & \textbf{OlympiadBench} & \textbf{Avg.} \\
% \midrule
% Random Masking &82.41&51.00&14.54&49.32        \\
% PPL‐based Masking        & \textbf{84.46}          & 51.2         & 14.99                 & 50.22         \\
% Gradient‐based Masking   & 83.09&\textbf{51.80}&\textbf{20.77}&\textbf{51.88}         \\
% \bottomrule
% \end{tabular}
% \end{table}

\begin{figure}[t]
  \begin{minipage}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/masking_strategy.pdf}
    \caption{Comparison of accuracy improvement with masking strategies over baseline (KD).}
    \label{fig:masking_strategy}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/splitting_strategy_.pdf}
    \caption{Comparison of accuracy improvement with splitting strategies over baseline (KD). }
    \label{fig:splitting_strategy}
  \end{minipage}
\end{figure}

\subsection{Response Splitting Strategies}
\label{sec: response_split_strategy}
We compare three response splitting strategies, considering that distracting patterns exist at both the instruction and response levels. We evaluate response without split (instruction-level pruning), 2-segment splits, and 3-segment splits. A diagram illustrating these strategies is shown in Figure~\ref{fig:instruct_cot_level_explain}. 
\paragraph{Results.}
As shown in the results in Figure~\ref{fig:splitting_strategy}, our findings are as follows: (1) Response-level pruning (both 2-segment and 3-segment splits) significantly outperforms instruct-level pruning, demonstrating the importance and benefits of extending the learning of confounding tokens from the instruction level to the response level. We hypothesize that the improvement stems from differences in distracting patterns between the instruction and response levels, suggesting that combining both levels could further enhance model performance. (2) The performance of 3-segment splits is comparable to that of 2-segment splits, suggesting that further segmentation at the response level yields diminishing returns. We hypothesize that distracting patterns at the response level exhibit certain regularities, and the data generated by 2-segment splits is sufficient for the model to learn these patterns effectively, rendering additional segmentation unnecessary.
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\textwidth]{Figures/instruct_mislead_explain.pdf} % 修改路径为你的图片路径
%     \caption{Illustration of Response Splitting Strategies: Language CoT, Instruct-level Masking, and Response-level Masking (2-segment and 3-segment splits). Highlighted white areas represent the input, and \textcolor{blue}{\underline{blue underlined areas}} represent the outputs used for cross-entropy loss computation.}
%     \label{fig:instruct_cot_level_explain}
%     % \vspace{-0.7cm}
% \end{figure}


% \begin{table}[t]
%   \centering
%   \caption{Comparison of output splitting strategies on reasoning benchmarks.}
%   \label{tab:split_comparison}
%   \small % 根据需要可以改成 \footnotesize
%   \begin{tabular}{lrrrr}
%     \toprule
%     Splitting Strategy & GSM8K & MATH & Olympiad & Avg. \\
%     \midrule
%     Output split 1/2 & 84.69 & 52.40 & 22.55 & 53.21 \\
%     Output split 1/3 & 84.00 & 52.40 & 20.92 & 52.44 \\
%     \bottomrule
%   \end{tabular}
% \end{table}

\subsection{Threshold Sensitivity Analysis}
\label{apex:threshold}
We perform a sensitivity analysis on the threshold used for confounding tokens pruning, assessing the performance of LLaMA3.2-1B-Instruct and LLaMA3.2-3B-Instruct as student models. As illustrated in the Figure~\ref{fig:llama_instruct} and Figure~\ref{fig:llama_step}, we present the average experimental results of these models across MathBench (GSM8K, MATH-500, OlympiadBench) at different threshold levels.

\begin{figure}[t]
  \begin{minipage}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/llama_instruct.pdf}
    \caption{Instruct-level in MathBench.}
    \label{fig:llama_instruct}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/llama_step.pdf}
    \caption{Response-level in MathBench. }
    \label{fig:llama_step}
  \end{minipage}
\end{figure}

\paragraph{Results.} We observe the following results:
(1) Instruct-level: LLaMa3.2-LeaF-1B performs best at a threshold of 0.10, while LLaMa3.2-LeaF-3B performs best at 0.05.
(2) Response-level: LLaMa3.2-LeaF-1B performs best at 0.15, and LLaMa3.2-LeaF-3B at 0.10.
(3) For both instruction-level and response-level, LLaMa3.2-LeaF-1B achieves optimal performance at a higher misleading token threshold than LLaMa3.2-LeaF-3B. This suggests that smaller models, which are more susceptible to confounding tokens, benefit from higher thresholds that filter out disruptive tokens more effectively.
Detailed cross-domain results presented in Appendix~\ref{app:threshold} further confirm that $\tau_{\text{mis}}=0.10$ yields stable performance across tasks.

\subsection{Case Study in an Interpretable Perspective}
\label{sec:case_study}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.8\textwidth]{Figures/case.png} % 修改路径为你的图片路径
%     \caption{
%     }
%     \label{fig:case_study}
% \end{figure}
We conduct a case study from an interpretability perspective to show that LeaF, compared to standard knowledge distillation (KD), enables the model to focus on critical information and avoid confounding tokens. The interpretability case study is shown in Figure~\ref{fig:case_study_analysis}. 
\begin{figure}[t!]
    \centering
    \includegraphics[width=1\textwidth]{Figures/case_study_new.pdf} % 修改路径为你的图片路径
    \caption{Case study comparing LeaF and knowledge distillation (KD) performance on the MATH-500. \textbf{Top:} Heatmap showing the attention score differences between KD and LeaF on instruction tokens. \textcolor{blue}{Dark blue} indicates higher KD attention, and \textcolor{pink}{deep pink} indicates higher LeaF attention. 
    %LeaF focuses more on tokens like “\textbf{\textcolor{pink}{multiple}}”, “\textbf{\textcolor{pink}{5}}”, and “\textbf{\textcolor{pink}{common fraction}}”. 
    \textbf{Left:} Response of LLaMA-3.2-3B-Instruct after standard knowledge distillation, with \textcolor{blue}{blue} text marking incorrect steps by the KD model. \textbf{Right:} Response of LLaMA-3.2-LeaF-3B, with \textcolor{pink}{pink} text highlighting correct steps by our model.
    }
    \label{fig:case_study_analysis}
    % \vspace{-0.5cm}
\end{figure}
It illustrates that LeaF allows the model to focus more on the critical information, such as "real number", "all", "are real". By identifying the requirement that all roots be real, LeaF guides the model through a coherent reasoning chain: recognizing $x = -1$ as an evident real root, and applying the discriminant condition to ensure the quadratic factor also yields real solutions. In contrast, the KD model overlooks this constraint and misapplies the AM--GM inequality to potentially negative values, resulting in an incorrect final answer. This demonstrates that LeaF enables the model to focus on critical information better.

% It illustrates that LeaF allows the model to focus on the core of the problem, such as the critical information "multiple" and "5" (combinations like (1,5), (2,5), etc.), which align with the condition "product of two numbers is a multiple of 5." In contrast, the KD model, due to insufficient attention to "multiple" and "5," initially focuses on "multiple of 5" but later incorrectly considers invalid combinations (e.g., 6 and 3), leading to an inaccurate final result. This demonstrates that LeaF enables the model to focus on critical information better.

==> hhcfmqnhvcmhjgxhytsngfvvpqzcbcgv/sections/06_related_work.tex <==
\section{Related Work}

% \textbf{Reasoning Consistency.} 
% A series of existing works have focused on decoding-phase consistency. Self-Consistency~\cite{wangself} stabilizes final answers by sampling multiple reasoning chains and applying majority voting. To further reduce inference costs, Adaptive Consistency~\cite{aggarwal2023let} and Early Scoring Self-Consistency~\cite{liescape} introduce Dirichlet-based and window-based stopping criteria, respectively. Reasoning Aware Self-Consistency~\cite{wan2024dynamic} enhances answer consistency by weighting sample quality and reasoning-path importance. 
%=
% However, these methods primarily focus on stabilizing the final answer without addressing the model's ability to maintain and leverage key contextual information throughout the generation process.
% %=
% We instead define consistency as both answer stability and context adherence, and introduce a distillation strategy that systematically suppresses the influence of misleading signals, enhancing the student's focus on key contextual information and promoting more robust context adherence during inference. 


\textbf{Chain-of-Thought Knowledge Distillation.}  
Our work falls within the knowledge distillation paradigm~\cite{hinton2015distilling,rule_distill}, a widely adopted technique for boosting the performance of open-source models in complex tasks such as mathematical problem-solving~\citep{zhu2024distilling,zhu2024improving} and code generation~\citep{ahmad2025opencodereasoning,huang2023program}.
%=
CoT-KD~\cite{shridhar2023distilling} takes the first step towards this line to employ chain-of-thought explanations generated by a high-capacity teacher to fine-tune a student model, thereby equipping it with advanced reasoning capabilities.
%=
Recent advancements can be broadly categorized into two complementary directions: 
%=
(1) \textbf{Data-focused approaches} aim to enhance distillation by improving the quality and diversity of training data (e.g., CD~\cite{feng2024teaching}, SCORE~\cite{zhang2024score}, and Skintern~\cite{liao2025skintern}).
%=
(2) \textbf{Model-focused approaches} enhance model architectures and inference strategies to improve efficiency and reasoning capability (e.g., PRR~\citep{shridhar2023distilling} and ATM~\citep{chen2024distilling}).
%=
However, existing methods primarily focus on output imitation, while our approach explicitly distills the teacher's ability to capture critical information during inference into the student, enabling context-aware reasoning in the student model.

\textbf{Critic Token Identification.}  Existing works have explored various strategies to identify and mitigate redundant steps~\citep{ding2024break,liu2024can,ma2025cot} or less-important tokens~\citep{han2024token,xia2025tokenskip} during language model reasoning. 
Methods like LLMLingua~\cite{jiang2023llmlingua} rely on models' self-assessment to determine token importance, which may introduce biases due to the model's limited reasoning capacity. 
%=
More recent approaches further refine token selection across different training stages. 
%=
RHO-1~\cite{lin2024rho} introduces Selective Language Modeling (SLM) during the Supervised Fine-Tuning phase, prioritizing informative tokens to enhance efficiency and reasoning accuracy. 
%=
TokenSkip~\cite{xia2025tokenskip} focuses on Chain-of-Thought stages, selectively skipping low-impact tokens to compress reasoning paths without sacrificing performance. 
%=
Meanwhile, cDPO~\cite{lin2024cdpo} enhances Direct Preference Optimization by isolating critical tokens through contrastive learning. 
%=
However, these methods primarily concentrate on output tokens while overlooking the influence of prior contextual information from the instruction phase. 
%=
In contrast, our method introduces an advanced teacher model to identify confounding tokens based on gradient differences, establishing stronger connections between instruction and output, and achieving more holistic and effective token filtering.

% \textbf{Reasoning Consistency.} Further discussion is provided in Appendix~\ref{app:relatedwork}.
\textbf{Reasoning Consistency.} A detailed discussion of reasoning consistency is provided in Appendix~\ref{app:relatedwork}.


==> hhcfmqnhvcmhjgxhytsngfvvpqzcbcgv/sections/08_conclusion.tex <==
\section{Conclusion}
In this paper, we proposed Learning to Focus Framework (LeaF), a novel strategy to enhance the consistency of large language models. By leveraging causal analysis and gradient-based pruning, our method effectively identifies and eliminates confounding tokens, enabling the student model to capture more reliable causal dependencies. Experimental results show substantial improvements in both accuracy and robustness across mathematical reasoning, code generation and multi-hop QA benchmarks. In future work, how to achieve model consistency through self-improvement mechanisms without relying on advanced models remains a promising direction for further exploration.

==> hhcfmqnhvcmhjgxhytsngfvvpqzcbcgv/sections/acknowledgments.tex <==
\section*{Acknowledgements}
This work was supported by The National Natural Science Foundation of China (No. 62376273 and No.U2436209) and Beijing Nova Program (No. 20240484568).

We sincerely thank all the anonymous reviewers and (S)ACs for their constructive comments, as well as Zhen Tian, Tingchen Fu, Wentong Chen, Yongda Yu, Hongjia Liu and Qinghui Wang for their valuable discussions on both the development of the ideas and the writing of this paper.


==> prompts/evaluation_code_prompt.tex <==
\begin{prompt}{Evaluation Prompt}
\label{prompt: evaluation_prompt}
The following is a math problem and a solution.
\\
The solution is presented as a step-by-step chain of thought.
\\
Each step is separated with the index indicator ``Step i:'', with i indexed starting from 1.
\\
\\
<Problem>
\\
\{problem\}
\\
</Problem>
\\
\\
<Solution>
\\
\{tagged\_response\}
\\
</Solution>
\\
\\
Your task is to evaluate the solution and identify the earliest step that contains an error, or confirm that all steps are correct.
\\
Please first review and generate a critique for each step.
\\
After reviewing each step, once you identify an error in the step, stop the critique and return the index of that step as this is the step where the earliest error occurs. Otherwise, continue reviewing the subsequent steps. If all steps are correct, return the index of -1 (which typically denotes ``not found'').
\\
Finally, put your final answer (i.e., the step index) in \verb|\|boxed\{\}.
\end{prompt}

==> sections/03_method.tex <==
\section{Methodology}
\subsection{Causal Framework}

Following Pearl's Structural Causal Model~\cite{pearl2010causal}, we formulate a DAG $G$ to model the causal relationships among different components (refer to Figure~\ref{fig:causal_graph}). We assume the distribution of $(X, A, Y)$ is faithful to the DAG. In this framework,  \( X = [x_1, x_2, \dots, x_n] \) represents the input tokens, and $Y$ is the model's output. Confounding tokens, denoted as $A$, are a subset of $X$ that introduce spurious correlations during reasoning. Unlike regular tokens that convey semantic information, confounding tokens hide the true causal relationship, leading to incorrect predictions. To better understand the DAG, we construct two hypotheses to describe the influence of confounding tokens $A$ on the generation process of $Y$:
\begin{wrapfigure}{r}{0.48\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{Figures/Causal_graph.pdf}
\setlength{\abovecaptionskip}{-0.8em}  
    \caption{Causal graph of the reasoning process. $X$ represents the input prompt, and $Y$ denotes the model's output. A subset of tokens in $X$, identified as confounding tokens ($A$), introduces spurious correlations that disrupt the reasoning process. Our method detects and masks $A$, effectively eliminating the spurious edge from $A$ to $Y$ and restoring the true causal dependency.}
    \label{fig:causal_graph}
    \vspace{-1.18cm}  
\end{wrapfigure}
\paragraph{$\mathcal{H}_0$: There is no causal edge from $A$ to $Y$.}
In this scenario, $A$ does not interfere with the generation of $Y$, and the model's reasoning path is purely determined by the meaningful tokens in $X \setminus A$. Formally, $A$ and $Y$ are \textbf{d-separated}
given $X \setminus A$, 
% (i.e., all paths from any token in \(A\) to \(Y\) are blocked once we condition on \(X \setminus A\))
which implies:
\begin{equation}
    P(Y \mid X) = P(Y \mid X \setminus A).
\end{equation}

% \paragraph{$\mathcal{H}_1$: There is a spurious correlation between $A$ to $Y$.}
\paragraph{$\mathcal{H}_1$: There is a nonzero causal edge from \(A\) to \(Y\).}
Equivalently, \(A\) and \(Y\) are not d-separated given \(X \setminus A\), which implies
\[
P(Y \mid X) \;\neq\; P\bigl(Y \mid X \setminus A\bigr).
\]
In this case, $A$ interfere with the output $Y$ by introducing erroneous correlations. This spurious dependency not only distorts the model's attention but also biases its output, leading to unreliable predictions.

% \subsection{d-Separation and Causal Inference}

The desired behavior of the model is to \textbf{remove the spurious correlation} of $A$ on $Y$, which corresponds to $\mathcal{H}_0$. To achieve this, we utilize the following d-separation properties in the DAG $G$:

\paragraph{R1: Under $\mathcal{H}_0$, $A$ and $Y$ are d-separated by $X \setminus A$.}
This implies that, conditional on the meaningful tokens in $X$, the confounding tokens $A$ should have no direct or indirect effect on $Y$:
\begin{equation}
    A \perp Y \mid (X \setminus A).
\end{equation}

\paragraph{R2: Under $\mathcal{H}_1$, $A$ and $Y$ are not d-separated by $X$, leading to spurious influences.}
In traditional LLM reasoning, these spurious paths can be exploited, causing the model to rely on distracting patterns. To eliminate this dependency, our method introduces \textbf{causal pruning}, effectively removing the influence of $A$ before distillation. This enables the distillation process to focus on the true causal pathways, refining the attention mechanism in the student model.

\subsection{\texttt{LeaF}: Learning to Focus Framework}
\label{sec:LeaF}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\textwidth]{Figures/main_.pdf} % 修改路径为你的图片路径
    \caption{\textbf{Method Overview.} The training pipeline comprises two key stages: (1) \textbf{Confounding Token Detection}: gradient-based comparisons between an advanced teacher model and the student model are used to identify confounding tokens (confounders) in the training corpus; and (2) \textbf{Causal Attention Distillation}: prune identified confounders respectively during training to align the student’s attention with the teacher’s and capture casual relationships. This targeted intervention steers the model toward actual causal dependencies, enhancing both robustness and interpretability.}
    \label{fig:main}
    \vspace{-0.3cm}
\end{figure}

To achieve the desired d-separation and eliminate spurious dependencies, we introduce a \textbf{Learning to Focus Framework (LeaF)} (Figure ~\ref{fig:main}), which consists of two main stages:  
(1) Confounding Token Detection (Section~\ref{misleading_tokens_detection}) and (2) Causal Attention Distillation (Section~\ref{causal_attention}). We discuss them in detail in the following.

\subsubsection{Confounding Token Detection} \label{misleading_tokens_detection}
To identify the confounding tokens $A$ that introduce spurious correlations, we adopt a \textbf{gradient-based approach}~\citep{simonyan2013deep,sundararajan2017axiomatic} to quantitatively measure the influence of each token on the model's output $Y$. 
%=
Specifically, we leverage the gradient sensitivity of both the teacher model $\boldsymbol{\theta}_T$ and the student model $\boldsymbol{\theta}_S$. 
%=
We focus on data instances mispredicted by the student but correctly handled by the teacher to isolate confounding tokens.
%=
For each token $x_i \in X$, we compute the gradient of the loss with respect to that token for both models:
\begin{equation}
    g^{(T)}_i = \left| \frac{\partial \ell(x_i \mid X; \boldsymbol{\theta}_T)}{\partial x_i} \right|, 
    \quad 
    g^{(S)}_i = \left| \frac{\partial \ell(x_i \mid X; \boldsymbol{\theta}_S)}{\partial x_i} \right|.
\end{equation}
These gradients reflect the sensitivity of each model to perturbations in $x_i$.
%=
To enable token-level comparison between models with differing gradient scales, we apply min-max normalization to the sensitivity values.
\begin{equation}
    \hat{g}^{(T)}_i = \frac{g^{(T)}_i - \min_j g^{(T)}_j}{\max_j g^{(T)}_j - \min_j g^{(T)}_j}, 
    \quad 
    \hat{g}^{(S)}_i = \frac{g^{(S)}_i - \min_j g^{(S)}_j}{\max_j g^{(S)}_j - \min_j g^{(S)}_j}.
\end{equation}
To identify confounding tokens, we capture the difference in token-level attention between the teacher and student models by computing the gradient difference for each token:
\begin{equation}
    \Delta \hat{g}_i = \hat{g}^{(T)}_i - \hat{g}^{(S)}_i.
\end{equation}
% To ensure consistency in the scale of gradient differences across all samples, we normalize the gradient difference \( \Delta \hat{g}_i \) as follows:

% \begin{equation}
% \hat{\Delta \hat{g}}_i = \frac{\Delta \hat{g}_i - \min_j \Delta \hat{g}_j}{\max_j \Delta \hat{g}_j - \min_j \Delta \hat{g}_j}.
% \end{equation}
To ensure consistent scaling of gradient discrepancies across instances, we normalize the gradient difference and classify a token \( x_i \) as a \textbf{Confounding Token} if (i) it receives significant attention from the student model but negligible attention from the teacher during inference, as formalized in Equation~\ref{eq:confounder_threshold}, and (ii) its removal results in correct predictions from both models.
\begin{equation}
\label{eq:confounder_threshold}
\frac{\Delta \hat{g}_i - \min_j \Delta \hat{g}_j}{\max_j \Delta \hat{g}_j - \min_j \Delta \hat{g}_j} \leq \tau_{\text{confounder}},
\end{equation}
where \( \tau_{\text{confounder}} \) is a threshold determined via statistical analysis on a validation set. Sensitivity analyses on the threshold are presented in Section~\ref{apex:threshold}.
%=
Intuitively, confounding tokens capture sensitivity discrepancies between the teacher and student models that indicate spurious dependencies.
%=

Moreover, we also explored perplexity-based detection, but without teacher guidance, it tends to capture tokens indicative of model uncertainty rather than true confounders, especially on challenging tasks like the Olympiads. Accordingly, we adopt gradient-based detection as our primary strategy (see Section~\ref{sec:masking-analysis} for details).
% We also explored PPL-based methods for identifying confounding tokens.
% However, without supervision from a stronger teacher, PPL tends to capture tokens reflecting model uncertainty rather than true confounders (especially in complex task like Olympiad). accordingly, we adopt gradient-based detection as our primary strategy (see Section~\ref{sec:masking-analysis} for details).
% We also explored PPL-based methods for identifying confounding tokens.
% However, without supervision from a stronger teacher, PPL tends to capture internal confusion rather than true distracting patterns—especially on difficult datasets like Olympiad.
% Thus, we adopt the gradient-based approach as our main strategy (see Section~\ref{sec:masking-analysis} for details).

% \paragraph{Causal Attention Distillation} 

 
% \paragraph{Causal Attention Distillation}
\paragraph{Pruning Strategies.}
We study two pruning strategies for removing confounding tokens from instruction \(X\): (1) \textbf{Collective Pruning}, which removes the entire set of identified confounders \(A\), yielding \(X \setminus A\).
(2) \textbf{Span Pruning}, which removes only one contiguous confounding span \(A_i\) at a time, yielding \(X \setminus A_i\). 
%=
Preliminary experiments show that span pruning outperforms collective pruning (see Appendix \ref{apex:separate}), as pruning all distracting patterns simultaneously disrupts sentence integrity. Hence, we construct the augmented dataset via the span pruning strategy:
%=
\[
\mathcal{D}_{\mathrm{pruned}}
= \bigl\{(X \setminus A_i, y)\bigr\}_{i=1}^{k},
\]
where each \(A_i\) denotes a distinct confounding span. This augmentation encourages the model to learn reasoning paths invariant to specific confounders. 
\begin{figure}[t!]
    \centering
    \includegraphics[width=1\textwidth]{Figures/span_masking.pdf} % 修改路径为你的图片路径
    \caption{Illustration of Collective Pruning and Span Pruning.}
    \label{fig:span_masking}
    % \vspace{-0.7cm}
\end{figure}
\subsubsection{Causal Attention Distillation} 
\label{causal_attention}
After generating both original and counterfactual samples, we optimize two complementary distillation objectives to steer the student toward true causal dependencies:

\textbf{Standard Distillation.} align the student’s output distribution with the teacher’s on original instructions:
\[
\mathcal{L}_{kd} = D_{\mathrm{KL}}\bigl(p_T(y\mid X)\,\|\,p_S(y\mid X)\bigr),
\]
where $p_T$ and $p_S$ denote the teacher and student output distributions, respectively.

\textbf{Counterfactual Distillation.} align the student’s output distribution with the teacher’s on counterfactual instructions $X\setminus A$ (confounders pruned):
\[
\mathcal{L}_{cd} = D_{\mathrm{KL}}\bigl(p_T(y\mid X\setminus A)\,\|\,p_S(y\mid X\setminus A)\bigr).
\]
we blend these objectives with a weighting factor $\lambda$:
\[
\mathcal{L} = \lambda\,\mathcal{L}_{kd} \;+\; (1-\lambda)\,\mathcal{L}_{cd},
\]
where $\lambda\in[0,1]$ controls the trade-off between standard and counterfactual distillation. This composite loss steers the student to preserve semantic knowledge while enforcing genuine causal dependencies.

\paragraph{Response Splitting Strategies.} For our methods, we consider two variants: (1) \textbf{Instruct-level Pruning}: We detect and mask confounding tokens only in the instructions, and perform our LeaF on the instruction-level masked samples. (2) \textbf{Both Instruct- and Response-level Pruning}: We can also treat previously generated tokens as contextual input, and mask those that are misleading for subsequent generation, in order to help the model produce more accurate continuations. Thus, we detect and prune confounding tokens in both instructions and preceding generations.

\begin{figure}[htp]
    \centering
    \includegraphics[width=1\textwidth]{Figures/instruct_mislead_explain.pdf} % 修改路径为你的图片路径
    \caption{Illustration of Response Splitting Strategies: Language CoT, Instruct-level Pruning, and Response-level Pruning (2-segment and 3-segment splits). Highlighted white areas represent the input, and \textcolor{blue}{\underline{blue underlined areas}} represent the outputs used for cross-entropy loss computation.}
    \label{fig:instruct_cot_level_explain}
    % \vspace{-0.7cm}
\end{figure}


% preliminary experiments (Appendix~\ref{apex:separate}) show that span pruning outperforms collective pruning.

% \paragraph{Pruning Strategies:} 
% We compare two pruning strategies (Figure~\ref{fig:span_masking}): (1) \textbf{Collective Pruning}, which simultaneously masks all identified confounding tokens. (2) \textbf{Span Pruning}, which masks only contiguous spans of tokens.

% After identifying the confounding tokens $A$ (confounders) that induce spurious dependencies, we construct a pruned instruction representation $X_{\backslash A}$ by removing them from $X$. This operation effectively eliminates spurious paths from $A$ to $Y$ in the causal graph. 
% %=

% Preliminary experiments show that span pruning outperforms collective pruning (see Appendix \ref{apex:separate}), as masking all distracting patterns simultaneously disrupts sentence integrity. Hence, we generate multiple pruned perturbations via the span pruning strategy:
% \[
% \mathcal{D}_{\text{masked}} = \{(X_{\backslash A}, Y), (X_{\backslash A'}, Y), (X_{\backslash A''}, Y), \dots\}
% \]
% where $A', A''$ represent distinct distracting patterns within the instruction.  This augmentation encourages the model to learn reasoning paths invariant to specific confounders. 

%通过Preliminary experiments，我们发现span pruning achieves superior performance than collective pruning for the reason masking all distracting patterns disrupts sentence integrity, resulting in suboptimal training signals. Thus, we generate multiple pruned perturbations by span pruning strategy:
%=
% To better preserve semantic integrity, we treat continuous confounding tokens as complete distracting patterns. 
%=
% Preliminary experiments indicate that each misleading pattern separately, rather than collectively, achieves superior performance (see Appendix\ref{apex:separate} for details).
%= 
% We hypothesize that simultaneously masking all distracting patterns disrupts sentence integrity, resulting in suboptimal training signals. Thus, we generate multiple masked perturbations by separately masking each misleading pattern:
% To enhance robustness, we generate multiple perturbations of the masked tokens:

% where $\lambda \in [0, 1]$ balances the influence of standard and pruning-based distillation. This composite loss function drives the student model to learn both robust semantic dependencies and causal consistency. 
% \paragraph{Mixed Distillation Training with Causal Interventions} 
% To operationalize our causal intervention strategy, we integrate two types of samples for distillation: 
% \textbf{(1) Standard Knowledge Distillation Data}: These are conventional distillation samples where the student learns from the teacher's soft labels:
% \begin{equation}
%     \mathcal{L}_{KD} = D_{\text{KL}}(p_T(y \mid X) \parallel p_S(y \mid X)),
% \end{equation}
% where $p_T$ and $p_S$ denote the teacher and student output distributions, respectively. This standard knowledge distillation approach is widely adopted for improving smaller models' performance and thus serves as the baseline in our experiments.

% \textbf{(2) Counterfactual Distillation}: These are the samples generated by tokens pruning introduced above, where confounding tokens are removed from the instruction:
% \begin{equation}
%     \mathcal{L}_{LeaF} = D_{\text{KL}}(p_T(y \mid X_{\backslash A}) \parallel p_S(y \mid X_{\backslash A})).
% \end{equation}
% Here, $X_{\backslash A}$ reflects the counterfactual scenario where spurious dependencies are eliminated, allowing the student to learn purely causal paths.




